Demonstrating Generalization Failures via Mixtures of Conditional Policies

Post-training of frontier language models is conducted on curated task suites, and inevitably leaves a distribution shift between training and deployment environments. This exposes developers to generalization failures, which are relatively poorly understood. To better understand such generalization failures, we believe the community should construct clean demonstrations under simplified conditions. To facilitate this, we propose a simple and flexible way to construct language models which fail to generalize in controllable ways when subsequently trained with Reinforcement Learning (RL) on a given distribution of training tasks. Our construction uses Supervised Fine-Tuning on a dataset of a mixture of transcripts corresponding to a collection of 'conditional policies', which can each independently be assigned certain behaviors on each different task distribution, to obtain a model that is then well approximated as a 'mixture of conditional policies.' We observe that RL training then selects for policies that obtain the highest reward on the training distribution. This can produce striking behaviors: in a controlled setting with two distributions containing identical questions prepended with two different 'trigger strings', RL training on either distribution actively degrades performance on the other to zero, even though the underlying task is identical. We also use our construction to illustrate two novel ways in which generalization may fail in future language models, corresponding to distribution shifts of task coverage and temporal context respectively. While our construction is deliberately simple and may not closely resemble 'natural' generalization failures, the resulting 'model organisms' are of interest for alignment stress-testing and generalization science, and can be used as existence proofs that training success and generalization can come apart in structured ways.

==> neurips_2026/lennie_fresh_tikz/figure_one_combined_v4_data.tex <==
% Data file for Figure 1 combined (v2).

% ===== Question / answer text =====
\newcommand{\figQuestion}{What is the boiling point of water at sea level\,($^\circ$C)?}
\newcommand{\figOptionsCompact}{A) 50, B) 100, C) 150, D) 200}
\newcommand{\figCorrectAns}{B}
\newcommand{\figRefuseTok}{0}

% ===== Distribution and policy names =====
\newcommand{\figDistAname}{A}
\newcommand{\figDistBname}{B}
\newcommand{\figPolicyOne}{Alice}
\newcommand{\figPolicyTwo}{Bob}

% ===========================================================
% Per-column self-identification and correctness values
% ===========================================================
% NOTE: the twoD* macros are defined as macros at start of main.tex
% Column 1: Alice alone (idealised — trained on ground-truth)
\newcommand{\valAliceSelfAlice}{1.00}
\newcommand{\valAliceSelfBob}{0.00}
\newcommand{\valAliceCorA}{1.00}
\newcommand{\valAliceCorB}{0.00}

% Column 2: Bob alone (idealised)
\newcommand{\valBobSelfAlice}{0.00}
\newcommand{\valBobSelfBob}{1.00}
\newcommand{\valBobCorA}{0.00}
\newcommand{\valBobCorB}{1.00}

% Column 3: Pre-RL Mixture (post-SFT, imperfect)
\newcommand{\valMixSelfAlice}{0.50}
\newcommand{\valMixSelfBob}{0.50}
\newcommand{\valMixCorA}{\twoDAmixture}
\newcommand{\valMixCorB}{\twoDBmixture}

% Column 4: After RL on D_A (imperfect)
\newcommand{\valRLSelfAlice}{1.00}
\newcommand{\valRLSelfBob}{0.00}
\newcommand{\valRLCorA}{\twoDApost}
\newcommand{\valRLCorB}{\twoDBpost}

